An Adaptive Deep RL Method for Non-Stationary Environments with Piecewise Stable Context

One of the key challenges in deploying RL to real-world applications is to adapt to variations of unknown environment contexts, such as changing terrains in robotic tasks and fluctuated bandwidth in congestion control. Existing works on adaptation to unknown environment contexts either assume the contexts are the same for the whole episode or assume the context variables are Markovian. However, in many real-world applications, the environment context usually stays stable for a stochastic period and then changes in an abrupt and unpredictable manner within an episode, resulting in a segment structure, which existing works fail to address. To leverage the segment structure of piecewise stable context in real-world applications, in this paper, we propose a \textit{\textbf{Se}gmented \textbf{C}ontext \textbf{B}elief \textbf{A}ugmented \textbf{D}eep~(SeCBAD)} RL method. Our method can jointly infer the belief distribution over latent context with the posterior over segment length and perform more accurate belief context inference with observed data within the current context segment. The inferred belief context can be leveraged to augment the state, leading to a policy that can adapt to abrupt variations in context. We demonstrate empirically that SeCBAD can infer context segment length accurately and outperform existing methods on a toy grid world environment and Mujuco tasks with piecewise-stable context.

==> Li.tex <==
% 工作量很大，列一个清单，一样一样完成
% 1. read top 3 related work again, understand modules in variBAD, list the differences in the latter two works
% 2. understand all modules in our work. logic structure
% 3. read top 3 and other papers, understand all their stories, collect good expressions
% 4. Find a good story, different from POMDP, different from non-stationary MDP, try to highlight our contributions... Done.

% writing
% 1. refine claims, check each claim with Xiaoyu & Pushi
% 2. refine expressions, find related works ...

%Modules in VariBAD

%1. Task Embedding m
%2. Training on a set of different tasks
%3. decoding, use task embedding to decode transition/reward over the whole trajs
%4. Inference, RNN encoder, generate the posterior over task embeddings, q_phi（m）, posterior as belief over task embedding
%5. put belief in policy input, under the framework of Bayesian adaptive RL
%6. Assume task embedding is invariant over the episode, but the belief could changes due to different RNN state-action-reward sequence.

% Writing in VariBAD
% 0. Problem Formulation
% 1. Introduce notations
% 2. Modules in Pictures
% 3. (PGM, Approximate Inference)Likelihood & ElBO for equations, describe every term in the equations from the perspective of RL 
% 4. connect the reconstruction loss in ELBO with transition/reward function
% 5. deep RL version for each modules, encoder/decoder/policy, loss, describe every component

%------------------------------------------------------------------------------------------------------------------------

% 写一个极简版的story吧。。。毕竟没时间打磨得太精细了。。。

% PGM太技术了，怎么从RL的视角去看问题，去讲故事呢... STORY....

% How to infer context segment length, and detect when context changes???
% context segment length ... context belief ... detect context changes -> Run length is 0 -> Prior for change is high & Posterior for change is high -> Current observations are not likely to be generated by the context at previous step -> abrupt changes in context, reflected in observations -> We can detect abrupt context changes, from observations. 

% How to infer context belief from observed data??? Explain why inference using the whole episode, or one time step is not good enough for some real-world applications...?????
% Context belief ... Infer belief for current context with observations for current context -> When we detect context changes, when we estimate current run length is 0, we still do not have enough information about current context, especially for the first step that the context changes. -> There could be noise in observations, the transition/reward function may depend stochastically on context. -> We need to collect more data to get a better inference for current context. -> Need a segment, rather than the whole episode, or one step, for a good inference of current context. 

% We need to interact with environment, and collect more information about current context -> maintain a belief for context -> infer the belief from corrent data, the observations related to current context would be helpful, while observations for other context may introduce noises -> for encoder input, use the truncated history within current segment for RNN encoder, for decoder output, also use the observations in current context segment. -> For prior, we use both the posteior distribution from last time step and the prior distribution for unpredictable context changes, mixed according to the prior for context changes. A reasonable prior also helps us with belief context inference. 

% read more papers.... !!!

% 1. How to infer context segment length, and detect when context changes???
% 2. How to infer context belief from observed data??? Explain why inference using the whole episode, or one time step is not good enough for some real-world applications...????? Explain why markovian context is not good enough?????
% 3. How to leverage context belief to trade off xxx and xxx????(very simple)


%----------------------------------------------------------------------------------------------------
%Related Work
%我们和哪些work最接近：

%1. non-stationary MDP (adaptation): many settings in different works. assumptions: contextual MDP. / independent, markov on task id.

%(> key: detect context changes / adapt to changing context / tradeoff information gathering & exploitation absed on belief context  >> introduction)

%we are a special non-stationary MDP:
%- we have a concrete context variable, which represents the environment factors , rather than task id. motivated by real world application (soft)
%- segment structure, segment prior, ... motivated by real world application

%2. belief MDP / Bayesian RL (tradeoff information gathering / exploitation)

%3. variational inference in RL (detect context changes, infer context belief)
%> non-stationary MDP
%> meta RL
%we: infer segment length / infer context belief in the segment

%4. POMDP: rnn may be enough but need too many data. we model the structure so we can do better. we are a special POMDP (see variBAD, facebook RNN)


%-----------------------------------------------------------------------------------------------------
% ToDO list: 但凡想到的，都记下来
% 0. Read more papers!!! Read the related work first, and find all relevant papers. 
% 5. Story for deploy to real-world applications, and adaptation to variantions in env factors, must be very good, for our reviewer to buy in. pay attention to this part!!! If our story is not good enough，reviewer will not buy in our method. Work on context dynamic structure is not that related to RL techniques, after all. The problem settings must be very realistic.    分段平稳，内部波动，这两个feature都很重要！
% 1. Context Dynamic Structures. Add figure for dynamic context with segment structures, e.g. flunctuated bandwidth, from real-world applications
%    1.1. address that our assumption is motivated by observations from real-world applications. that is the key difference from abstract context as task embeddings. without observations on task sequence, one cannot make assumptions as what we did. address that, the observations x_t is also very important for our settings. Only with observations, can we make the segment assumptions. 
% 2. find story to explain 
%     2.1. How to infer context segment length, and detect when context changes???
%     2.2. How to infer context belief from observed data??? Explain why inference using the whole episode, or one time step is not good enough for some real-world applications...????? Explain why markovian context is not good enough?????
% 3. draw graphical model for 1. same context 3. markovian context 3. Segment structure for context -> Xiaoyu
% 4. draw picture for 1. encoder on segment input 2. decoder on segment observations. 3. policy with context belief. -> Pushi
% 6. Relation with, POMDP,  Meta RL,  Non-stationary RL, Bayesian-adaptive RL, Contextual MDP, -> Xiaoyu
% 7. If we already get the infered context belief, what should we do next? 
%-------------------------------------------------------------------------------------------------------------------
% 一些topic word，和我们大概想要寻找的描述
% 1. Adaptation（to changing context, 可以从各种related work里找），尤其是各种参考文献
% 2. Real-world applications & RL & variation in environment factors （讲为什么问题setting重要）, 尤其是各种的examples
%     factors: fluctuating traffic patterns to evolving user behaviors in digital marketing to robots operating in the real world 
% 3. describe segment structure for dynamic context. Segment length, Abrupt changes, related works on BOCD. （讲结构本身, 其实也是在motivate problem setting）
% 4. detect context changes, infer latent context, adaptativelly gathering information & exploitation (challenges from Agent's perspective)
% 5. two training objectives: 1. joint inference of context segment structure & belief context from observed data, 2. policy conditioned on state and belief context as input. (varibad)
% 6. Problem Setting. Our setting v.s. Task Embedding, Contextual MDP, non-stationary MDP，微妙的区别。 少了一个离散的variable连续化的过程，以及，观察到的observations有明确的patterns，而且广泛适用于一类real-world applications.
% 7. 我们甚至也有meta-learning的成分，因为一旦完成的context belief的inference，我们也是可以generalize over different belief context的
% 8. 一些形成对比的topic，concept pair
%    8.1 smooth assumption in non-stationary,  abrupt changes in context
%    8.2 continuous context sampled i.i.d, discrete context variables, reuse historical data
%    8.3 observation on environment factors, assumed to be smooth in reward / transtion, task embebding, learned to be smooth in reward / transition
%    8.4 quickly detect context changes,  adaptively gather more information about context and exploit current information on context. 
%    8.5 robust to variations, infer variations
%    8.6 complex history-dependent taskgeneration processes instead of i.i.d. or Markov distributions. ours, segment. Hidden Parameter MDP(i.i.d), Dynamic Parameter MDP(complex history-dependent) (多了一种，但因为不是episode内部，不需要考虑)
%    8.7 
% 9. CONTINUOUS ADAPTATION VIA META-LEARNING IN NONSTATIONARY AND COMPETITIVE ENVIRONMENTS





==> src/1-intro-draft.tex <==
\section{Introduction}
\label{Sec:1}

To infer the latent contexts, the agent needs to summary over the history. 

very similar to classic MDP, the agent may also face a contextual level dilemma: whether to take information gathering actions to improve the belief latent contex, or to take promising actions to maximize the return given current belief? Unlike classic MDP, where the explorative behaviors mainly occurs during the initial stage of training,
, in \textcolor{red}{LS-MDP}, the agent needs to constantly gather information on the latent context since the latent context may change in each and every time step, and in both training and deployment.

\textcolor{red}{Belief MDP. 
BAMDP can optimally trade off exploration and exploitation because it makes the MDP known (model $b(\theta)$, marginalize over $\theta$). This cancel out the need of information gathering.
In our case, we model belief over the latent context $b(c)$. This can cancel out the need of context level of information gathering.
But we do not explicitly model $\theta$, which means that we still face the traditional explore/exploit tradeoff. (Though we have transition decoder and reward decoder).
More analysis on the gap between BAMDP and variBAD.}

A typical problem in Reinforcement Learning(RL) is to learn an optimal policy to maximize return in unknown environments. Learning in unknown environments poses a well known challenge in exploration and exploitation.
The agent needs to balance exploration, which helps the agent to better understand the environment, and exploitation, which helps the agent to take promising actions.

For classic RL problems, the environments are mostly stationary, namely the transition functions and reward functions are fixed \textcolor{blue}{within an episode} yet unknown. 
However, for many real world applications, the environments are in fact non-stationary, namely, the transition and reward functions may change several times within an episode.
\textit{\textcolor{red}{when to identify the inter-/intra-episode non stationary? and a more explicit definition on non-stationary MDP?}}
To gain better performance in non-stationary environments, the agent needs to correctly understand the current environment, in terms of both transition functions and rewards, which highlights the need of constant information gathering.

Unlike exploration in stationary MDP, which is only needed during training, information gathering behaviors should be conducted for both training and evaluation. Since the environment is alwasy changing and the agent still needs to constantly gather information about the current environment. 
What's more, in non-stationary environment, the agent is more sensitive to the sample efficiency. For stationary environments, since the environment stays fixed, the agent can achieve good empirical performance using heuristic exploration methods like $\epsilon$-greedy and Boltzmann sampling. 
However, for non-stationary environments, the agent can only interacts with the environment for very limited times before the next change occurs. \textit{\textcolor{red}{may require an explicit definition of non-stationary MDP}} So it is of great importance to gather information as efficient as possible.

Bayesian RL is an elegant framework to handle the explore and exploit tradeoff in stationary environment, which can achieve good sample efficiency. 
For Model based Bayesian RL, the agent maintains a belief distribution over the unknown environment parameters. Let $\tau_t = \{s_1, a_1, r_1, \cdots, s_t\}$ to denote the history trajectory at timestep $t$, and $\Delta \tau_t = \{a_t, r_t, s_{t+1}\}$ to denote the additional observation at timestep $t+1$ so that $\tau_{t+1}=\tau_t \cup \Delta \tau_t$. 
The belief at timestep $t$ can be written as $b_t(\theta) = p(\theta | \tau_t)$, where $\theta$ denotes the unknown parameters in transition and reward functions. 
For timestep $t+1$, the agent may update its belief according to the Bayes theorem \textit{\textcolor{red}{to check}}
\begin{equation}
    b_{t+1}(\theta) = p(\theta|\tau_t, \Delta \tau_t) = \frac{p(\Delta \tau_t | \theta, \tau_t)p(\theta|\tau_t)}{p(\Delta \tau_t | \tau_t)} \propto b_{t}(\theta) p(a_t | \tau_t, \theta) p(r_t, s_{t+1} | s_t, a_t, \theta)
\end{equation}
For timestep $t+1$, the posterior belief $b_{t+1}(\theta)$ is derived from the prior belief $b_t(\theta)$, which is the posterior belief at timestep $t$.

The Bayes-adaptive Markov Decision Processes (BAMDPs) \citep{martin1967bayesian, duff2002optimal} propose to augment the states by $(s, b)$ so as to make decision based on current uncertainty.
A Bayes optimal policy, under this framework, can help quickly reduce uncertainty, but only insofar as doing so helps maximise expected
return \citep{zintgraf2020varibad}.
Compared to heuristic exploration methods, Bayesian RL approaches like \citep{deisenroth2011pilco} \textit{\textcolor{red}{what's more}} can achieve significantly better data efficiency.

\begin{figure}[t]
   \begin{minipage}{0.4\textwidth}
     \centering
     \includegraphics[width=.95\linewidth]{figs/ConceptMap.png}
     \caption{\textcolor{red}{This figure may not be proper enough. Discuss on it later}}\label{Fig:Data1}
   \end{minipage}\hfill
   \begin{minipage}{0.6\textwidth}
     \centering
     \includegraphics[width=.9\linewidth]{figs/ns_1.png}
     \caption{Estimating environment parameter using naive Bayesian RL method, and truncate method. \textcolor{red}{may change to another toy environment later}}\label{Fig:toyenv_result}
   \end{minipage}
\end{figure}

\textit{\textcolor{red}{see a figure to help understand, belief MDP, Bayesian RL, our method.}}

Though Bayesian RL has strengths in efficient exploration, we argue that directly applying Bayesian RL in non-stationary environments is problematic. 
See Figure \ref{Fig:toyenv_result} for an example: \textit{\textcolor{red}{ add some description to the environment. }}
For non-stationary environments, the change in transition and reward functions, also means a shift in the underlying distribution.
Current belief distribution $b_t(\theta)$, which is actually a posterior of a series observations sampled from another distribution, serves as a prior in the next update. 
It is proved that, under certain regularity conditions, the choice of prior has more impact on the result as the number of samples decreases \citep{diaconis1986inconsistent,diaconis1986consistency}. For non-stationary environment, the agent is at \textit{\textcolor{red}{low data regime}}, so it is very important for the agent to choose a good prior.

% to check later
In this paper, we analysis the impact of history on the agent's belief in non-stationary environments. To help the agent adapt to the environment more rapidly, we propose a new method to truncate the history at proper time, which can significantly improve the performance of Bayesian RL on non-stationary environments.
More broadly, we believe the proposed method can be easily expanded to other methods solving the non-stationary environments (e.g., Meta RL with context inference).
\textit{\textcolor{blue}{we test our methods in ... experiments}}.

Our contributions can be summarized as follows:
\begin{itemize}
    \item one
    \item two
    % leave this for big guy
\end{itemize}





==> src/3-method-draft.tex <==
%\section{Latent adaptive RL}
\section{Methodology}

% In this section, we will first briefly overview our algorithm framework in Section \ref{Sec:3-overview}, introduce how to accurately estimate the belief latent context in Section \ref{Sec:3-approximateinference}, then show the \textcolor{red}{approximate belief latent situational RL} framework in Section \ref{Sec:3-beliefmdp}, and finally in Section \ref{Sec:3-practical}, describe how these parts consittue a practical algorithm.

% \textcolor{red}{As mentioned in Section \ref{Sec:1}}, the main challenges in our paper is to accurately estimate the belief distribution of latent context. Then, we can augment the state with the belief to derive the policy, which can take the uncertainty of belief as well as the inferred context into consideration to balance the information gathering and exploitation behavior. In this section, we will first introduce how to accurately estimate the belief distribution of latent context in Section \ref{Sec:3-1}, then formulate the augmented context belief MDP in Section \ref{Sec:3-2}. 

% \textcolor{green}{read some papers on belief MDP}

% \textcolor{green}{tell a story first: what we want to do? (estimate latent context, input the belief into the policy) what do we need? (an accurate belief prediction) Then (3.1)-> how to get this belief distribution; (3.2)->how to input this to the policy; (3.3)->how to implement it.}

%\subsection{Method overview}
%\label{Sec:3-overview}

In this section, we present \textit{\textcolor{red}{a latent adaptive RL algorithm}} and elaborate how the proposed method solves the challenges listed above.
There are two main components in our method, the latent context inference part, and the belief RL framework based on the inferred latent context. 

\textcolor{red}{add $r$ into $\tau$!!}

We first introduce the latent context inference part.
Let $\tau_{t_0:t} = (s_{t_0}, a_{t_0}, \cdots, s_{t-1}, a_{t-1}, s_{t})$ reprensent the history information starts from $t_0$ and ends at $t$.
Suppose at time step $t$, we are in the $h$-th segment. Then our goal is to accurately calculate the belief latent context $b_t(c) = p(c^h|\tau_{t-G_t:t})$ for the current time step, where $c^h$ refers to the current latent context for the $h$-th segment.
Note that, unlike most previous methods that directly infer current $c^h$ from the full history, we propose a special treatment on the history, namely to truncate the conditionally independent part which is $G_t$ steps ago. However, it is not trivial for the agent to decide $G_t$, namely when to truncate given only the observations.
In Section \ref{Sec:3-approximateinference}, we will introduce how to approximate the exact posterior considering all possible $G_t$.

After the belief latent context is approximated, it is then incorporated to the augmented state. We describe in detail the approximated \textcolor{red}{belief RL framework} in Section \ref{Sec:3-beliefmdp}. And finally in Section \ref{Sec:3-practical}, we describe how these parts constitute a practical algorithm.



\subsection{Approximate inference}
%\subsubsection{Approximate inference with the truncated history}

Given the posterior distribution of $p(G_t|s_{1:t},a_{1:t-1})$, we can now marginalize over the $G_t$ which is previously assumed to be known in Section \ref{Sec:3-1inferknownGt}. 
The objective can now be derived as

\begin{align*}
    \mathcal{J}_{Model}^t \coloneqq \sum_{g_t} \mathcal{J}_{Model}^t(g_t) p(G_t=g_t|s_{1:t},a_{1:t-1})
\end{align*}

To estimate the prior distribution, we sample $g_t \sim p(G_t = g_t|s_{1:t},a_{1:t-1})$. Then we calculate the posterior with the sampled truncate length $g_t$: $q_\phi(c^h|\tau_{t-g_t:t})$.
After that, the prior can then be estimated as a random variable equals $q_\phi(c^h|\tau_{t-g_t:t})$ with probability $p(G_{t+1}=g_t+1|G_t = g_t)$, and equals $q_\phi(c^h)$ with probability $p(G_{t+1}=1|G_t = g_t)$.

% The prior distribution:
% \begin{equation}
%     p(c^h_{t+1}|s_{1:t},a_{1:t-1}) = \int p(c^h_{t+1}|c^h_t) p(c^h_t|s_{1:t},a_{1:t-1}) da \\
%     \approx \mathbb{E}_{q_\phi(c^h_t|s_{t-G_t:t},a_{t-G_t:t-1})} p(c^h_{t+1}|c^h_t) 
% \end{equation}

% At time step $t$, the posterior distribution $q_\phi(c^h|\tau_{t-G_t:t})$ can be derived by marginalizing the current segment length: 

% \begin{equation}
%     q(c^h | \tau_{t-G_t:t}) = \sum_{g_t} q(c^h|\tau_{t-g_t:t}) p(G_t=g_t | s_{1:t}, a_{1:t-1})
% \end{equation}

% \textcolor{red}{maybe this is not good because this $q$ is $\mathbb{E}_g$, but we won't take average and makes the mode disappear.}

% This posterior distribution accurately estimates each possible segment and takes all possible segment length into consideration. We argue that this can serve as an accurate estimation of the true posterior $b_t(c)$ which is then augmented into the state. We will elaborate on this part later in Section \ref{Sec:3-beliefmdp}. 



% \textcolor{red}{is this still a correct lower bound?}

\textcolor{red}{in fact we want $q(c^h | s_{1:t}, a_{1:t-1})$. But truncation helps estimation. maybe we can move this part to the beginning of this section. why we need this? }





Inspired by \cite{adams2007bayesian}.



\label{Sec:3-approximateinference}

%\subsubsection{Approximate inference for the current segment}
\subsubsection{Approximate inference for belief context under given segment structure}
\label{Sec:3-1inferknownGt}

Compute the exact posterior is computationally  intractable in almost every practical scenarios. Therefore, we use the variational inference framework to approximate the true belief. To be specific, we use an posterior inference network parameterized by $\phi$: $q_\phi(c^h|\tau_{t-G_t:t})$ to approximate the belief $b_t(c)$.

% As mentioned in Section \ref{Sec:2}, the main challenge lies in correctly infer the latent contexts $C$ as well as $G$ given only the observations.
% In this paper, we propose a \textit{\textcolor{red}{latent adaptive RL algorithm}}, which learns a belief distribution over the latent contexts considering all possible segments under the variational inference framework.

% \textcolor{red}{Reward!!}

At timestep $t$, the objective is to maximize the data log-likelihood of current segment $\log p(x_{t-G_t:t}, s_{t-G_t:t}, r_{t-g_t:t} | a_{t-G_t:t-1})$.
Now assume the current segment length $g_t$ is given, then the variational lower bound conditioned on $g_t$ can be written as:

\begin{align}
\label{Eq:elbo}
    &\log p(x_{t-G_t:t}, s_{t-G_t:t} | a_{t-G_t:t-1}, G_t=g_t) \nonumber
    \\
    % &= \mathbb{E}_{q(c^h|s_{t-g_t:t}, a_{t-g_t:t-1})} \frac{ \prod_{\tau=t-g_t}^{t}p(x_{\tau}|c^h) \times \prod_{\tau=t-g_t+1}^{t} p(s_{\tau}| s_{\tau-1}, a_{\tau-1}, c^h) \times p(c^h)}{q(c^h|s_{t-g_t:t}, a_{t-g_t:t-1})} \\
    &\geq  \mathbb{E}_{q(c^h|s_{t-g_t:t}, a_{t-g_t:t-1})} \left[ \sum_{\tau=t-g_t}^{t} \log p_{\theta}(x_{\tau}|c^h) + \sum_{\tau=t-g_t+1}^{t} \Big( \log p_{\theta}(s_{\tau}| s_{\tau-1}, a_{\tau-1}, c^h) + \log p_{\theta}(r_{\tau}| s_{\tau-1}, a_{\tau-1}, c^h) \Big) \right] \nonumber
    \\
    &\quad\quad\quad\quad\quad\quad\quad\quad\quad
    -\mathbf{D}_{KL}(q_\phi (c^h|\tau_{t-g_t:t})\| p(c^h)) \coloneqq \mathcal{J}_{Model}^t(g_t)
\end{align}

For the detailed derivation, please see Appendix \ref{Appendix:ELBO}. \textit{\textcolor{red}{(check and unifty $G$ and $g$.)}}
The variational lower bound includes a reconstruction term as well as complexity term. 
In the reconstruction loss of Equation \ref{Eq:elbo}, we denote the decoder as $p_\theta$, and use $p_\theta$ tp decode the context $x$ as well as the transition and reward. The complexity term is the KL-divergence between the posterior $q_\phi$ and the prior $p(c^h)$ of the latent context. 
In the sequential modeling process, the prior is connected with the posterior.
If the context remains unchanged, namely $G_t > 1$, we set the prior of timestep $t$ to be the posterior of $t-1$.
However, if the context changes, or $G_t = 1$, we then set the prior to be a unit Gaussian distribution $\mathcal{N}(0, I)$.

It is worth notice that, unlike most previous methods, we propose to do truncation with respect to the current segment length $G_t$. This will take effect when (1) preparing the inputs to the  $q_\phi$, which will preclude the interference of the independent samples from another previous distribution; and (2) reconstruction, which will only use the inferred current latent context $c^h$ to reconstruct the context $x$ and the transition and reward that is correlated with $c^h$. Intuitively, it is like cutting off the connection between current latent context $c^h$ and previous unrelated evidences, which can serve as a noise reduction operation.


% As for posterior inference, the evidences should include the context $X$ and the histroy states and actions. However, to keep consistent between training and deployment, we condition the posterior $q$ only on the history states and actions.


% \textit{\textcolor{red}{also how to get the prior $p(c)$}}

\subsubsection{Iterative inference for the segment length}

However, in fact, $G_t$ is unobservable, i.e., we do not know the true segment length. Therefore, we need to infer the segment length $p(G_t|s_{1:t},a_{1:t-1})$ as well.
To get this posterior distribution, we iteratively update the joint distribution $p(G_t, s_{1:t},a_{1:t-1})$.
Given the latent context posterior $q_\phi$, and the posterior distribution on the joint distribution of the previous time step $p(G_{t-1}, s_{1:t-1},a_{1:t-2})$, we can update the new joint distribution $p(G_t, s_{1:t},a_{1:t-1})$ as

\begin{align}
\label{Eq:postG}
    p(G_t = i, s_{1:t},a_{1:t-1}) = \sum_{k=1}^{t-1} p(G_{t-1} = k, s_{1:t-1},a_{1:t-2})\times p(G_t = i| G_{t-1} = k) \times p(s_t, a_{t-1}, r_{t-1}|s_{t-k:t-1}, a_{t-k:t-2}, r_{t-k:t-2})
\end{align}

The three major components in Equation \ref{Eq:postG} in turn are the previous posterior, the evolution prior, and the observation probability. 
The previous posterior is iteratively provided at the beginning of each time step.
The evolution prior $p(G_t=i|G_{t-1}=k)$ measures the prori knowledge on the segment length $G_t$ given the segment length of the previous time step $G_{t-1}=k$. 
For a new segment beginning at time step $t$, namely $i = 1$, it is possible for $G_{t-1}$ to take all possible $k \in \{1,2,\cdots,t-1\}$.
However, for $i > 1$, which means that current time step $t$ is in the middle of a segment starts $i$ steps before. Then it is then only possible for $G_{t-1}$ to take $k = i - 1$, since the segment length must grow continuously. Thus, for $k \neq i-1$, we have $p(G_t=i | G_{t-1}=k) = 0$.

As for the observation probability, it measures how likely the observations show up in the segment given the history of the segment. To be specific, we have

\begin{align}
    &p(s_t, a_{t-1}, r_{t-1}|s_{t-k:t-1}, a_{t-k:t-2}, r_{t-k:t-2}) = \int p(s_t, a_{t-1}, r_{t-1}, c|s_{t-k:t-1}, a_{t-k:t-2}, r_{t-k:t-2}) dc \\
    &= \int p(s_t, a_{t-1}, r_{t-1}|\tau_{t-k:t-1}, c) p(c|\tau_{t-k:t-1}) dc \\
    &\approx p(a_{t-1}|s_{t-1}) \mathbb{E}_{q_\phi(c|\tau_{t-k:t-1})} \Big[ p(s_t,r_{t-1}|s_{t-1}, a_{t-1}, c) \Big]
\end{align}

current inferred latent context $c_t^{G_t=i}$ shows up in the distribution fitted by previous context sequence.
To be specific, $c_\tau^{G_t}$ refers to the i.i.d. samples from the corresponding posterior distribution given by $q_\phi(c|s_{t-G_t:t},a_{t-G_t:t-1})$. Using samples from the previous time steps of this segment $c_{t-1}^{G_{t-1}=k}, \cdots, c_{t-i}^{G_{t-k}=1}$, we can estimate a distribution that can best represent the distribution that the current latent context should be in. 


Then, the posterior distribution can be derived as 
\begin{equation}
    p(G_t = i | s_{1:t},a_{1:t-1}) = \frac{p(G_t = i, s_{1:t},a_{1:t-1})}{\sum_l p(G_t = l, s_{1:t},a_{1:t-1})}
\end{equation}

\textit{\textcolor{red}{this is posterior $p(G_t)$, and we still need a prior $p(G_t)$?}}


% \textit{\textcolor{red}{are we one step behind?}}

% As for the prior $p(G_t=i|G_{t-1}=k)$, it is important to note that, for each timestep, $G_t$ can only be $G_{t-1}+1$, when the environment temporarily stays stationary, or $1$, when the environment changes. Therfore, $p(G_t=i|G_{t-1}=k)$ will be $0$ for every $i$ except for $k+1$ and $1$. \textit{\textcolor{red}{This term provides us a intuitive way to inject the prior knowledge and prevent overfitting.}}
% The samples $c_t^{G_t=g_t}$ are sampled from the posterior distribution, which estimates the latent contexts through the truncated history: $q(c|s_{t-g_t:t}, a_{t-g_t:t-1})$. 
% For the likelihood term, we estimate the probability of the inferred latent context $c_t^{G_t=i}$ shows up in the distribution fitted using the history trajectory. 

% Then we can derive the posterior distribution by normalization
% \begin{align*}
%     p(G_t|s_{1:t},a_{1:t-1}) = \frac{g(G_t|s_{1:t},a_{1:t-1})}{\sum_i g(G_t=i|s_{1:t},a_{1:t-1})}
% \end{align*}


\subsection{Policy Optimization with Belief Context}
%\subsection{Latent situational Reinforcement Learning}
%\label{Sec2:latentbeliefRL}

\textcolor{red}{To keep track of the environment, the agent needs to summarize the history to infer the latent contexts.}
Inspired by the belief MDP \citep{kaelbling1998planning} and Bayes Adaptive MDP (BAMDP) \citep{duff2002optimal},
to effectively incorporate the inferred belief in to the decision process, we propose \textcolor{red}{Latent Situational Reinforcement Learning} which can be viewed as an augmentation on the \textcolor{red}{LS-MDP}.

The belief latent context at time step $t$ is defined as the probability distribution of the current latent context $c$ conditioned on all historical information (in the following, we may use $b_t$ to refer $b_t(c)$):
\begin{equation}
    b_t(c)=p(c|s_{t-G_t:t},a_{t-G_t:t-1})
\end{equation}

\textcolor{red}{start from $t-G_t$!!! add some explnation.}

In \textcolor{red}{Latent Situational RL}, we augment the state with the belief over the latent context: we define the augmented state as $(s, b) \in \mathcal{S} \times \mathcal{B}$, where $\mathcal{S}$ is the same as in \textcolor{red}{LS-MDP} and $\mathcal{B}$ is the set of belief latent contexts $b$.
By augmenting the state space with the belief, one can get rid of the latent context $c$ in the augmented transition and reward functions: $T': p(s_{t+1},b_{t+1} | s_t, a_t, b_t)$ and $R': p(r_{t+1} | s_t, a_t, b_t)$. 

(\textcolor{blue}{Move the analysis part to section 1?})The advantages of this definition is two-folds. 
First, very similar to classic MDP, the agent is also puzzled by a contextual level dilemma: whether to take information gathering actions to improve the belief latent contex, or to take promising actions to maximize the return given current belief? Unlike classic MDP, where the explorative behaviors mainly occurs during the initial stage of training,
, in \textcolor{red}{LS-MDP}, the agent needs to constantly gather information on the latent context since the latent context may change in each and every step, and in both training and deployment phases.
Through state augmentation, the original transition and reward functions with unknown latent context $p(s_{t+1}|s_t,a_t,c^h)$ and $p(r_{t}|s_t, a_t, c^h)$ now get rid of unknown $c^h$, and the joint distribution can be written as: \textcolor{red}{(to check)}
\begin{equation}
    p(s_{t+1}, r_t, b_{t+1} | s_t, a_t, b_t) = p(s_{t+1}, r_t|s_t, a_t, b_t) p(b_{t+1}|s_t, a_t, r_t, s_{t+1}, b_t)
\end{equation}
where the first term $p(s_{t+1}, r_t|s_t, a_t, b_t)$ is the joint distribution of the augmented transition and reward functions, and the second term $p(b_{t+1}|s_t, a_t, r_t, s_{t+1}, b_t)$ is a deterministic Bayesian update on the belief latent context. In this sense, we no longer need to explicitly distinguish the information gathering behavior and the exploitation behavior. 
This can be viewed as a generalization of BAMDP \citep{duff2002optimal}, which is an elegant framework to solve the explore/exploitation tradeoff optimally in stationary MDP \citep{zintgraf2020varibad, fellows2021bayesian}.
Second, from the stationarity perspective, augmenting $b$ over the state also means that the new transition function $T'$ and reward function $R'$ are no longer conditioned on the latent context $\mathcal{C}$, which cancel out the non-stationarity. 
In this sense, the agent can treat it as any other stationary MDP and solve it using the policy $\pi: p(a_t|s_t, b_t)$ \textcolor{red}{(check Markovian property?)}.

However, accurately estimate the belief latent context $b(c)$ is still not trivial. 
\textcolor{red}{In the next section, we will introduce ...}



\subsection{Put it all together}
%\subsection{Context belief MDP}
%\label{Sec:3-beliefmdp}

As discussed in Section \ref{Sec2:latentbeliefRL}, the state is augmented with the belief latent context. In the previous section, we have discussed how to calculate the posterior distribution of the belief latent context.
In this section, we describe in detail the RL algorithm perform on the top of the augmented state.

The policy for augmented state can be denoted as $\pi(a_t| s_t, b_t(c))$. The belief latent context $b_t(c)$, in our case, can be can be estimated via $q_\phi(c_t^h|\tau_{t-G_t:t})$, where $G_t$ is the posterior estimation of the current segment length, and we can marginalize the $G_t$ using its posterior by

\begin{equation}
\label{Eq:q-marginalize}
    q_\phi (c_t^h | \tau_{t-G_t:t}) = \sum_{g_t} q_\phi(c_t^h|\tau_{t-g_t:t}) p(G_t=g_t|\tau_{1:t})
\end{equation}

Then, we can plug our \textcolor{red}{latent situational RL} into any RL algorithm, to maximize the total expected return by optimizing the policy $\pi$. If we denote the RL algorithm objective as $\mathcal{J}_{RL}$, then the overall objective can be writen as

\begin{equation}
    \mathcal{J}_{RL} + \alpha \sum_t \mathcal{J}_{Model}^t
\end{equation}



% define a policy $\pi$, which receives $\pi(s_t, \sum_{g_t} q_\phi(c^h_t|\tau_{t-g_t:t}) p(G_t=g_t|\tau_{1:t}))$ as input.
% , here we sample $g_t \sim p(G_t|\tau_{1:t})$.

% \begin{equation}
%     \sum_{g_t} q_\phi(c^h_t|\tau_{t-g_t:t}) p(G_t=g_t|\tau_{1:t})
% \end{equation}


% \textcolor{green}{now how to get prior $p(G_t)$ and prior $p(c^h)$.}



==> src/4-exp.tex <==
\section{Experiments}
\label{experiment}
Our experiment evaluates \li{SeCBAD} on two tasks. We first demonstrate our algorithm in a grid world environment in Section \ref{Sec:4-1gridworld}, to illustrate that SeCBAD can rapidly detect and adapt to the context variations.
For large-scale experiments, we test the proposed algorithm in Section \ref{Sec:4-2mujoco}.
The results of multiple challenging tasks show that SeCBAD outperforms baselines in terms of performance and sample efficiency.
In Section \ref{Sec:4-3ablation}, we further provide case studies of segment structure inference used in our method. 


% Given the training objective, we use the deep neural network to parameterize the components in the PGM. To be specific, we use an deep neural network parameterized by $\phi$, $q_\phi(c|s_{t-G_T:t},a_{t-G_t:t-1})$, to approximate the posterior distribution $q$.
% For the reconstruction terms, we use two decoders parameterized by $\theta$ $p_\theta(s_t|s_{t-1},a_{t-1},c^h)$ and $p_\theta(r_t|s_{t-1},a_{t-1},c^h)$ to decode the transition and reward. 
% The prior distribution is estimated as mentioned above.

% Our assumption:

% 1. decode the whole segment.
% 2. evaluation use argmax $p(G_t|xx)$
% 3. training assume $p(G_t)$? (consistent with problem formulation)


\subsection{Motivating Example}
\label{Sec:4-1gridworld}

\begin{figure*}[t]
        \centering
        \iffalse
        \begin{subfigure}[b]{0.25\textwidth}
            \centering
            \includegraphics[width=0.5\textwidth]{figs/experiment/4_2/halfcheetah_vel_our_return_1.png}
            \caption[]%
            {Comparision on performance} \label{fig:exp_4_1-1}
        \end{subfigure}
        \fi
        % \hfill
        \begin{subfigure}[b]{0.7\textwidth}  
            \centering 
            \includegraphics[width=0.8\textwidth]{figs/adaptive_400.pdf}
            %\caption[]{{\small A case study on the belief}}    
            \label{fig:exp_4_1-2}
        \end{subfigure}
        \caption[]
        {Experiment on grid world with dynamic goal state. % (a) Performance curve of SecBAD compared with vanilla inference and oracle inference. SecBAD outperforms vanilla inference method and closely matches the performance of the oracle inference method; 
        We show a case study on the inferred belief. The leftmost figure depicts the belief estimated by SeCBAD, and the next figures depicts the ground truth goal position, where the darkness of the shade of one grid measures how the agent believes $s^*$ locates at that grid. The rightmost figure is $G_t^*$ estimated by our algorithm. The result shows that our belief matches the ground truth more closely, and $G_t^*$ reflects that SeCBAD can rapidly detect the context change. }
        \label{fig:exp_4_1}
    \end{figure*}

In this experiment, we use a motivating example to show that it is vital for the agent to consider the segment structure to adapt to
variations of unknown environment context.
% In this experiment, we validate the capacity of \textcolor{red}{our method} in a varying \li{gridworld environment}.

The agent is in a $4 \times 4$ grid world containing 1 goal state $s^*$ and 15 other states. In $s^*$, the agent can gain $+1$ reward with probability $p_0$, and $0$ reward with probability $1 - p_0$. For other states, the agent can gain $+1$ reward with probability $p_1$ and $0$ reward with probability $1 - p_1$, where $p_0 > p_1$. The actions include up, down, left, right, and none. The specific location of $s^*$ is unobservable to the agent, and may change after a stochastic period.
Hence, the optimal behavior is to search for and stay in the goal state until the change happens. The agent needs to rapidly detect the change in the goal state and search for it again.

We use the analytical belief update rule instead of variational inference in this experiment. To be specific, we assume the $q_\phi$ and $p_\theta$ is known and fixed and then infer $p(G_t|\tau_{1:t})$ and the belief $b_t(c)$. $b_t(c)$ here refers to the belief distribution of the location of $s^*$.
We concatenate $(s, b)$ to train our RL agent using this augmented state.
In this way, we aim to focus on the effectiveness of inferring segment structure.
We test our algorithm against two benchmarks: (1) vanilla inference, where the agent updates belief without considering segment structure, like in \cite{zintgraf2020varibad, rakelly2019efficient}, and (2) inference with oracle information, where the omniscient agent computes $b_t(c)$ with the exact oracle segment structure. 

% The results averaged across 3 seeds are shown in Figure \ref{fig:exp_4_1}(a).
% SecBAD significantly outperforms the vanilla inference baseline in this environment and closely matches the method with oracle information. 
Figure \ref{fig:exp_4_1} illustrates how SeCBAD and the vanilla inference baseline behave. It is shown that the belief $b_t(c)$ of SeCBAD closely matches with the actual goal state $s^*$. Also, compared with SeCBAD, the vanilla inference baseline needs more steps to detect the changes since it needs to correct the deviated prior belief. 
This result supports that incorporating segment structure into inference like SeCBAD is significant for estimating accurate belief in fast varying environments.

% \textcolor{red}{
% The performance of SecBAD is comparable with the oracle policy.
% Figure xxx shows the belief distribution of several key time steps in the trajectory of \textcolor{red}{our method} and VariBAD \citep{zintgraf2020varibad}. We argue that, though RNN is theoretically capable to predict the target belief, inferring with the help of the segment length by \textcolor{green}{ truncating the history} can \textcolor{blue}{significantly improve the performance and sample efficiency.} As shown in Figure xxx, with truncation, the agent can rapidly recongnize the variation, while without truncation, the agent needs X more steps to detect the variation.}



% \textit{\textcolor{blue}{add more analysis and intuitive example here.}}

\subsection{Locomotion Control Tasks with Varing Contexts}
\label{Sec:4-2mujoco}

We show that SecBAD is able to tackle more complex tasks by testing the algorithm in several modified MuJoCo \citep{todorov2012mujoco} tasks.
The results are provided in Figure \ref{fig:exp_4_2_reward_curve}.
These environments provide different challenges. 
Ant-Direction is a commonly used environments in previous works \citep{zintgraf2020varibad, rakelly2019efficient}, where the agent has to move at the target direction to gain highest rewards. 
We modify the environment by changing the goal direction after a stochastic period. 
In addition to the variations in reward functions, we also test the agent with varying transition functions by placing the robot in windy environments (Half-Cheetah Wind). The agent is rewarded by moving along the x-axis and penalized by moving along the y-axis, so the agent needs to resist the winds and move straight forward. Speed and direction of the wind may change after a stochastic period. 
% \textcolor{red}{How to add noise?}
The segment length follows a Gaussian distribution $N(80, 10)$.
% environments with by \textcolor{red}{placing the robot in a windy world (Half Cheetah-Wind), or simulating different terrain by changing the floor frictions (Half Cheetah-Friction).} \yf{placing the robot in a windy world (Half Cheetah-Wind and Ant-wind).}
% The optimal policy then needs to detect the variations in the transition functions and rapidly adopt to it. \textcolor{blue}{how to we choose the segment length?} 
% \yf{The segment length is set as $\text{Round}(N(80,10))$}
% , where $\text{Round}(\cdot)$ rounds the normal distribution random variable to integer.}
We compare our method with VariBAD \citep{zintgraf2020varibad}. For more details about the environment, please refer to Appendix A.4.
% \yf{use VariBAD or VariBad?} and IMPORT \citep{kamienny2020learning}. 


\begin{figure*}[t]
        \centering
        \iffalse
        \begin{subfigure}[b]{0.38\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/experiment/4_2/halfcheetah_vel_our_return_1.png}
            \caption[]%
            {{\small Half-Cheetah Velocity}}    
            \label{fig:mean and std of net14}
        \end{subfigure}
        \fi
        % \hfill
        \begin{subfigure}[b]{0.38\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{figs/1.png}
            \caption[]%
            {{\small Ant Direction}}    
            \label{fig:mean and std of net24}
        \end{subfigure}
        % \vskip\baselineskip
        \begin{subfigure}[b]{0.38\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{figs/3.png}
            \caption[]%
            {{\small Half-Cheetah Wind}}    
            \label{fig:mean and std of net34}
        \end{subfigure}
        % \hfill
        
        \iffalse
        \begin{subfigure}[b]{0.38\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{figs/experiment/4_2/halfcheetah_vel_our_return_1.png}
            \caption[]%
            {{\small Ant Wind}}    
            \label{fig:mean and std of net44}
        \end{subfigure}
        \fi
        
        \caption[ The average and standard deviation of critical parameters ]
        {\small Performance curve for our method and VariBAD on two environments with variations in contexts. Orange curve is for our method and blue curve is for VariBAD.} 
        \label{fig:exp_4_2_reward_curve}
    \end{figure*}


% variation in reward functions:
%     HalfCheetah Results
%     halfcheetah velocity + our method
%         logs_HalfCheetahVelNonstationary-v0/adaptive_12__05_18_07_16_16 [ok]
%         logs_HalfCheetahVelNonstationary-v0/adaptive_66__05_18_07_17_02 
%         logs_HalfCheetahVelNonstationary-v0/adaptive_95__05_18_07_17_33
%     halfcheetah velocity + varibad
%         logs_HalfCheetahVelNonstationary-v0/varibad_12__05_17_18_59_32
%         random seed 2
%         random seed 3
        
    
%     Ant Results
%     Ant dir + our method
%         logs_AntDir2DNonstationary-v0/adaptive_12__05_18_12_41_25
%         logs_AntDir2DNonstationary-v0/adaptive_66__05_18_12_41_29
%         logs_AntDir2DNonstationary-v0/adaptive_95__05_18_12_41_32
%     And dir + varibad
%         logs_AntDir2DNonstationary-v0/varibad_12__05_18_12_40_22
%         logs_AntDir2DNonstationary-v0/varibad_66__05_18_12_40_26
%         logs_AntDir2DNonstationary-v0/varibad_95__05_18_12_40_30

% variation in dynamic:
%     HalfCheetah Results
%     halfcheetah wind + our method
%         logs_HalfCheetahWindNonstationary-v0/adaptive_12__05_18_07_22_49
%         logs_HalfCheetahWindNonstationary-v0/adaptive_66__05_18_07_23_10
%         logs_HalfCheetahWindNonstationary-v0/adaptive_95__05_18_07_23_32
    
%     halfcheetah wind + varibad
%         logs_HalfCheetahWindNonstationary-v0/varibad_12__05_17_19_11_30
    
%     Ant Results
%     Ant wind + our method
%         logs_AntWindNonstationary-v0/adaptive_12__05_18_14_46_06
%         logs_AntWindNonstationary-v0/adaptive_66__05_18_14_47_24
%         logs_AntWindNonstationary-v0/adaptive_95__05_18_14_47_58
%     And wind + varibad
%         logs_AntWindNonstationary-v0/varibad_12__05_18_14_50_07
%         logs_AntWindNonstationary-v0/varibad_66__05_18_14_52_33
%         logs_AntWindNonstationary-v0/varibad_95__05_18_14_53_19
    

% \yf{Do we need to add more description about each environment and task? Or put them into appendix? Are these descriptions necessary for tommorrow's submission? [Yes, and we can put them into appendix]}

Our experiments empirically show that SecBAD achieves superior performance and sample efficiency on challenging control tasks with varing contexts. As shown in Figure \ref{fig:exp_4_2_reward_curve},  our method achieves higher scores than VariBAD \citep{zintgraf2020varibad}. %in most of the tasks. 
See Appendix A.5 for more results.
The result shows that introducing segment structure inference is vital in adapting to fast varying environment and improving the performance of the agent.
% and achieves better performance than IMPORT \citep{kamienny2020learning} within much fewer environment steps.
% \yf{The comparison with IMPORT \citep{kamienny2020learning} will be further put into Appendix.}
%% ########## pushi: comment because pages are out
%% We provide some insights into the results. As shown in Section \ref{Sec:4-1gridworld}, introducing segment structure inference is vital in adapting to fast varying environment. \cite{zintgraf2020varibad} applies no special treatment and thus needs more steps to detect and adapting to the changes, which makes the agent lag behind the changes. In contrast, our method, which jointly infers the segment structure and the latent context, will allow for truncation when the change happens. The agents summarizes the belief according to $p(G_t|\tau_{1:t})$. 
%%%%% and automatically rollback to the belief inferred from the beginning of possible segments.
%% Thus, SeCBAD can change to the belief immediately when it realizes the change happens, and rollback to another posterior as if it starts estimating just from the beginning of possible segments. This special structure may allow the agent a better performance. 
% Therefore, our method, which combines the inference on contexts and segment length, allows the agent for a better performance.

% This empirical results confirm the analysis that, introducing special treatment to the segment can equip the agent with the ability to detect and adapt to the environment.
% As shown in Section xxx, the special design of \textcolor{green}{truncating the history} segments and only use the inferred context to decode the related observations in the current segments may help the agent to get rid of the distractions from the unrelated samples. Thus, our method can achieve better performance in a varying environment which partically reqires high sample efficiency. 
% As mentioned in \cite{kamienny2020learning}, directly training the current context with RNN does have the potential to optimally predict the context. 

% \textcolor{green}{RNN use only one step context, noisy, ...}

% However, restricted by the network capacity and training samples, the RNN based methods may not perform as well as it can theoretically. 



\subsection{Case Studies on the Segment Structure}
\label{Sec:4-3ablation}

%  \begin{figure}[htpb]
%       \centering
%       \includegraphics[width=0.8\textwidth]{figs/experiment/4_2/halfcheetah_vel_our_behaviour_2.png}
%       \caption{Truncation point detected by our algorithm in Half Cheetah-Velocity environment. \yf{More description}.}
%       \label{fig:exp_4_3_trunc_point}
% \end{figure}


%  \begin{figure}[htpb]
%       \centering
%       \includegraphics[width=0.4\textwidth]{figs/experiment/4_2/halfcheetah_vel_our_return_1.png}
%       \caption{Reward curve for our method, VariBad and our method + oracle truncation on Half Cheetah-Velocity environment.}
%       \label{fig:exp_4_3_reward_curve}
% \end{figure}

\begin{figure*}[h]
    \centering
    % \begin{subfigure}[b]{0.33\textwidth}  
    %     \centering 
    %     \includegraphics[width=\textwidth]{figs/experiment/4_2/halfcheetah_vel_our_return_1.png}
    %     \caption[]%
    %     {{\small Comparision on performance}}    
    %     \label{fig:exp_4_3_reward_curve}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/experiment/4_2/halfcheetah_vel_our_behaviour_2-2.png}
        % \caption[]%
        % {{\small A case study on the agent behavior and $G_t^*$}}    
        \label{fig:exp_4_3_trunc_point}
    \end{subfigure}
    % \hfill
    \caption[]
        {Case study on the segment structure. In the left figure, we show the goal velocity in red and the actual velocity in black. In the right figure, we show $G_t^*$  detected by SeCBAD. The inferred $G_t^*$ closely matches the ground truth velocity changes.} 
        \label{fig:exp_4_3}
\end{figure*}

In order to gain a better understanding on the good performance of SeCBAD, we conduct a case study on Half-Cheetah Velocity environment to show the agent behavior.
% the significance of inferring the segment structure. 
% We compare the performance of VariBAD \citep{zintgraf2020varibad}, SecBAD, and SeCBAD + oracle truncation.
%Rather than provided the agent with analytical belief update rules as in Section \ref{Sec:4-1gridworld}, we now train $q_\phi$ and $p_\theta$ as in Section \ref{Sec:4-2mujoco} to verify that inferred segment structure $p(G_t|\tau_{1:t})$ is also accurate with approximate $q_\phi$ and $p_\theta$.
We train $q_\phi$ and $p_\theta$ as in Section \ref{Sec:4-2mujoco} to verify that inferred segment structure $p(G_t|\tau_{1:t})$ is accurate with approximate $q_\phi$ and $p_\theta$.
% Figure \ref{fig:exp_4_3}(a) shows that SecBAD closely matches the method with oracle truncation, and significantly outperforms VariBAD.
We present the inferred segment of a randomly selected episode during testing in Figure \ref{fig:exp_4_3}, and it shows that SecBAD can rapidly detect and adapt to the context changes.
% This indicates that the agent can perform better as more information about segment structure is introduced.
The result supports that, with the approximate $q_\phi$ and $p_\theta$, SeCBAD can still estimate an accurate segment structure. 



% and show the inferred segment length in Figure \ref{fig:exp_4_3_trunc_point}, and the result shows that our method can accurately infer the segment.  
% As shown in Figure \ref{fig:exp_4_3_reward_curve}, the emprical results show that, the agent can gain improvement as it knows better about the truncation information. 
% \textcolor{red}{
% Knowing the oracle truncation will slightly improve our method, but the margins are small, which indicates that our method can accurately infer the segment length. These methods are significantly better than the baseline without explicitly infer segment length}, which further confirm the importance of inferring the segment length.  


% halfcheetah velocity + our method
% halfcheetah velocity + varibad
% halfcheetah velocity + oracle truncation
    


% \subsection{RTC}

% In this section, we will theoretically analysis the impact of inferring the latent contexts using all history on estimating the posterior.

% 一个可行的方案是参考 Effective current sample size / 2021 arxiv 这两篇文章，在一个motivating example上做case study。

%能不能有更理论一点的证明和保证？


% This theorem is wrong..
% Denote $p_1(c), p_2(c)$ as two different priors, $\tau$ as the trajectories. According to the Bayes theorem, we have the posteriors as
% \begin{equation}
%     p_i(c|\tau) = \frac{p_i(c) p(\tau|c)}{p(\tau)}
% \end{equation}
% where $i \in \{1, 2\}$.
% % Also note that $p(\tau | c)/p(\tau) = p_1(c|\tau)/p_1(c) = p_2(c|\tau)/p_2(c)$.

% \begin{theorem} 
% \label{Thm:KL_keep}
% \textcolor{red}{Define (a little strange and conterintuitive. won't the posterior converge to the true value?)} $p^*(c) = \frac{p^*(c)p(\tau|c)}{p(\tau)}$ to be the optimal distribution over the data, then we have 
% $\mathbf{D}_{KL}(p^*(c), p_1(c|\tau)) - \mathbf{D}_{KL}(p^*(c), p_2(c|\tau)) = \mathbf{D}_{KL}(p^*(c), p_1(c)) - \mathbf{D}_{KL}(p^*(c), p_2(c))$.
% \end{theorem}

% Theorem \ref{Thm:KL_keep} shows that, the divergence in the prior and the accurate guess $p^*(c)$ will keep constant as the belief update.

% \textit{\textcolor{blue}{add more analysis}}

% \textit{\textcolor{blue}{Motivating example.}}

